Human languages order information efficiently

Most languages use the relative order between words to encode meaning relations. Languages differ, however, in what orders they use and how these orders are mapped onto different meanings. We test the hypothesis that, despite these differences, human languages might constitute different `solutions' to common pressures of language use. Using Monte Carlo simulations over data from five languages, we find that their word orders are efficient for processing in terms of both dependency length and local lexical probability. This suggests that biases originating in how the brain understands language strongly constrain how human languages change over generations.

==> Makefile <==
.PHONY: dvi ps pdf all space clean veryclean distclean

SHELL = /bin/sh
MAKE  = gmake

# latex --interaction {batchmode, nonstopmode, scrollmode, errorstopmode}
#TEX = latex --interaction batchmod
TEX = latex --synctex=1 -file-line-error-style
PDFTEX = pdflatex --synctex=1 -file-line-error-style

######################################################################
# source files

texfiles = $(wildcard *.tex)
bibfiles = $(wildcard *.bib)

tblfiles = $(wildcard tbl/*.tex)

styfiles  = $(wildcard *.sty)

figfiles  = $(wildcard img/*.tex)
figfiles += $(wildcard fig/*.plt)
figfiles += $(wildcard fig/*.pdf)
figfiles += $(wildcard fig/*.ps)
figfiles += $(wildcard fig/*.epsi)
figfiles += $(wildcard fig/*.c)

tmp_files = $(wildcard *.log)
tmp_files += $(wildcard *.aux)
tmp_files += $(wildcard *.blg)
tmp_files += $(wildcard *.toc)
tmp_files += $(wildcard *.dvi)
#tmp_files += (texput.log)

######################################################################
# output files

target = si

######################################################################
# make targets

all: pdf

dvi: ${target}.dvi

ps: ${target}.ps

pdf: ${target}.pdf

space:
	@if [ -d fig ]; then cd fig; ${MAKE} $@; fi
	@-/bin/rm -f ${tmp_files} *~ ${target}.pdf ${target}.ps

clean veryclean distclean:
	#	if [ -d fig ]; then cd fig; ${MAKE} $@; fi
	/bin/rm -f ${tmp_files} *~ ${target}.pdf ${target}.ps ${target}.dvi

######################################################################
# rules

%.dvi : %.tex ${figfiles}
	@${TEX} $<
	@if grep -q bibdata ${*F}.aux ; then \
		bibtex ${*F};	\
		${TEX} $<;	\
		bibtex ${*F};	\
	fi
	@${TEX} $<
#	@-/bin/rm -f ${tmp_files}

%.ps : %.dvi
	dvips -P pdf -G0 -q -o $@ $<

slides.pdf : slides.ps ${figfiles}
	ps2pdf $< $@

slides.test.pdf : slides.test.ps ${figfiles}
	ps2pdf $< $@

%.pdf : %.tex #${texfiles} ${bibfiles} ${styfiles} ${figfiles} ${tblfiles}
	@if [ -d fig ]; then cd fig; ${MAKE} all; fi
	@${PDFTEX} $<
	@${PDFTEX} $<
	@-/bin/rm -f ${tmp_files}


#%.bib:	%.aux
#	BSTINPUTS=/u/gildea/src/bibtools-2000/bibtools /u/gildea/src/bibtools-2000/bibtools/aux2bib $<
#	mv references.bib $@


slides.ps : slides.dvi
	dvips -t landscape -P pdf -G0 -q -o $@ $<


######################################################################
# dependences

${target}.dvi: ${texfiles} ${bibfiles} ${styfiles} ${figfiles} ${tblfiles} Makefile

